Cores and Other Dense Structures in Complex Networks

Complex networks are a powerful paradigm to model complex systems. Specific network models, e.g., multilayer networks, temporal networks, and signed networks, enrich the standard network representation with additional information to better capture real-world phenomena. Despite the keen interest in a variety of problems, algorithms, and analysis methods for these types of network, the problem of extracting cores and dense structures still has unexplored facets. In this work, we present advancements to the state of the art by the introduction of novel definitions and algorithms for the extraction of dense structures from complex networks, mainly cores. At first, we define core decomposition in multilayer networks together with a series of applications built on top of it, i.e., the extraction of maximal multilayer cores only, densest subgraph in multilayer networks, the speed-up of the extraction of frequent cross-graph quasi-cliques, and the generalization of community search to the multilayer setting. Then, we introduce the concept of core decomposition in temporal networks; also in this case, we are interested in the extraction of maximal temporal cores only. Finally, in the context of discovering polarization in large-scale online data, we study the problem of identifying polarized communities in signed networks. The proposed methodologies are evaluated on a large variety of real-world networks against na\"{\i}ve approaches, non-trivial baselines, and competing methods. In all cases, they show effectiveness, efficiency, and scalability. Moreover, we showcase the usefulness of our definitions in concrete applications and case studies, i.e., the temporal analysis of contact networks, and the identification of polarization in debate networks.

==> advisor.tex <==
Dear Ph.D. Symposium Chairs,

we certify that Edoardo Galimberti is a third year Ph.D. Student in good standing at University of Turin.
He has double affiliation as he is at both the Computer Science department of the University of Turin, and the ISI Foundation.
We strongly support his participation to the symposium since, at the current status of his research, he would benefit a lot from presenting the results obtained until now and receiving feedback about future and ongoing work.

Edoardo has obtained strong theoretical results since the beginning of his Ph.D. studies about dense subgraphs and cores in complex networks.
He has achieved two publications in a prestigious venue as CIKM, and has papers under review to The Web Conference and the TKDD Journal.
Currently, Edoardo is working onto two different research directions.
On one hand, he is enriching the theoretical results about temporal networks and, at the same time, experimenting the application of the developed tools for the analysis of spreading processes.
Moreover, he is participating in other parallel research projects, e.g., the LinkedIn Economic Research Challenge.

The anticipated date for thesis completion is December 2019, then he is plenty of time to put into practice all feedback and suggestions he will receive at the symposium.

\vspace{0.75cm}

\noindent Yours sincerely,

\noindent Giancarlo Ruffo, Ph.D.

\noindent Francesco Bonchi, Ph.D.

\noindent (the advisors)

==> student.tex <==
Dear Ph.D. Symposium Chairs,

I am Edoardo Galimberti, third year Ph.D. student at the Computer Science Department of University of Turin and researcher of the Algorithmic Data Analytics group at ISI Foundation.
My doctoral research is about the study of cores and dense structures in complex networks, with a particular focus on algorithmic aspects.

The purposes of attending the Ph.D. Symposiums of The Web Conference are several.
At first, I would love to receive direct feedback on my ongoing and future research from experienced researchers different than my colleagues at the University and ISI.
Any opinion from a completely different prospective can only enrich the quality of my work.
Secondly, I would like to present my research results and future plans to other Ph.D. colleagues, and attend their presentations.
This will also give me the possibility of discussing, debating, providing, and receiving feedback about my and other Ph.D. researches in a context of reciprocal knowledge.
Finally, I would appreciate to enlarge my network by exchanging ideas and experiences, and lay the foundations for future collaborations.
At this stage of my Ph.D. program, I am sure that I will fully benefit from attending the symposium and that it will be an enriching experience in many aspects.

The topics/questions that I would like to discuss with the mentors are the following:
\begin{itemize}
\item How can I complete my research from a theoretical standpoint? Which are the related topics that would deserve to be considered in the remaining of my Ph.D.?
\item Which real-world data can I model with the developed tools? How can I derive concrete applications?
\item Which is the amalgam of the research topics that I studied until now? What is missing to develop a flawless narration for my Ph.D. thesis?
\end{itemize}

\vspace{0.75cm}

\noindent Yours truly,

\noindent Edoardo Galimberti
